It Is Not Where You Are, It Is Where You Are Registered: IoT Location Impact

This paper investigates how and with whom IoT devices communicate and how their location affects their communication patterns. Specifically, the endpoints an IoT device communicates with can be defined as a small set of domains. To study how the location of the device affects its domain set, we distinguish between the location based on its IP address and the location defined by the user when registering the device. We show, unlike common wisdom, that IP-based location has little to no effect on the set of domains, while the user-defined location changes the set significantly. Unlike common approaches to resolving domains to IP addresses at close-by geo-locations (such as anycast), we present a distinctive way to use the ECS field of EDNS to achieve the same differentiation between user-defined locations. Our solution streamlines the network design of IoT manufacturers and makes it easier for security appliances to monitor IoT traffic. Finally, we show that with one domain for all locations, one can achieve succinct descriptions of the traffic of the IoT device across the globe. We will discuss the implications of such description on security appliances and specifically, on the ones using the Manufacturer Usage Description (MUD) framework.

==> abstract.tex <==
\begin{abstract}
In this paper, we investigate the network traffic of IoT devices. First, we show that, unlike general purposes devices (such as computers and smartphones), smart devices access only a few endpoints. %In the vast majority of cases, a DNS request to a specific domain precedes a connection to an endpoint. Thus, IoT traffic can be defined by the set of domain names the device connects with. 
In our dataset, the median number of domains each device connects to is 7 (range 1-68 domains).

%As IoT devices aim to connect to nearby services, an important research question is whether the set of domain names changes when the device is deployed in another region.  We have distinguished between two  IoT deployment locations: its physical location (based on Geo-IP) and its user-defined location (given by the user in the registration process). 
We have measured more than 30 IoT devices, each at up to 10 locations, and show that, surprisingly, the user-defined location is the major factor on the device's network behavior, while the physical location itself has almost no effect. 

Maintaining a set of domain names for every possible (user-defined) location puts a burden on security devices that use this set to monitor (and secure) IoT traffic. 
Hence, we suggest using Extended DNS, to simplify the network architecture of IoT devices, reducing the number of required domains. %In our scheme, the device requests the same domain name no matter what its user-defined location is (yielding a succinct set of domain names). With EDNS Client Subnet (ECS) field, the device can indicate its (user-defined) location, implying a resolver supporting ECS, will reply with an IP address that is close to the device's (user-defined) location. 
In our measurements, ECS is supported by 7 out of the 8 
most popular DNS providers, accounting for 86.20\% of the users of these providers.  
In addition, the ECS field is being forwarded (without modification) in every resolver we have checked. 


Finally, we show the properties of the set of domain names directly affect IoT security tools that use this set to detect malicious traffic. Specifically, the IETF Manufacturer Usage Description (MUD) framework generates an allowlist according to this set. We show how by using EDNS the number of entries in this allowlist (namely, the number of  ACLs) is significantly reduced and the entire MUD's allowlist management and deployment processes become more streamlined.  
\end{abstract}
%each device connects to only 13 domains on average.  MAX MIN. 

%  to defend the device is reduced and MUD is more conveniently supported.
%
%Specifically,    

%One of the fundamental research questions is what are the main factors that affect device network behavior; whether the physical location (based on Geo-IP) or the user-defined location (in the registration process) affects the device network behavior.

%We made measurements that were based on more than 30 IoT devices, captured in up to 10 locations, and found that the user-defined location is the main factor on the device's network behavior. Nonetheless, in opposition to the common theory, a device that is registered in the same place but physically located (IP-based location) in different places presents similar network behavior.

%different user-defined locations the device requests the same domain with a different Client-Subnet (ECS). Then, the device gets IP address correlated to the user-defined location. 
%In our measurements, we found that ECS is supported by 56.7\% of the resolvers in RIPE ATLAS machines. 
%


%86.20\% of the users that use open resolver, which are 60.65\% from all DNS users, use resolvers that support ECS and 

%In this paper, we show that the user-defined location, and not IP-based location, influences the domains that the device connects to; The same device connects different domains and sub-domains in different user-defined locations. It complicates the design, development and the security maintenance for the manufacturer. %, i.e., increasing the MUD adopting cost for the manufacturer. It also affects the IETF MUD standard, which assumes that each firmware has only a single MUD file for all available locations.

%Analyzing the network behavior of IoT devices, including which domains the device communicates with, is a fundamental challenge for IoT security and identification. %Solutions that analyze and manage these areas must be able to learn what constitutes normal device behavior and then extract rules and features to permit only legitimate behavior or to identify the device.
%We present a network architecture, leveraging the Extended DNS Client-Subnet option (ECS) to enhance IoT security design, decreasing maintenance costs and amount of required ACLs and support user-defined location. Our propsal allows a more convenient and secure way to describe the legitimate behavior of a device.

%ECS was designed to allow recursive resolvers, to forward details about the client network when questioning the authoritative name servers. Usually, it is used by content delivery networks when the client is not near the recursive resolver.As opposed to traditional implementations of ECS in which the authoritative adds ECS option. We suggest that the IoT device itself will add an ECS option, with the user-defined location. 
%This allows the manufacturer the flexibility needed to support locations separation with minimal costs, without requiring different domains per location. We found that 62\% of the resolvers support ECS and all of them forward it, from the client, to the authoritative. 
%Finally, we evaluate our proposal, comparing it to current proposals, in regards to amount of required ACLs and explainability for network administrators.

%We show experimental results that ECS has currently a high adoption rate in DNS resolvers and explain how ECS and logical location can be useful in other fields such as web-browsing. We present a scenario in which the use of ECS can give the required flexibility of user-configurable location.


%Cases decision is based on user defined location, example IoT.
%In this paper we show that it is common to use different domains to different locations.
%This complicate the maintenance and also has impact on MUD standard, that assume there is MUD file per firmware, and thus not support ...
%We show that EDNS, what is EDNS, that came to solve another problem,,,, .. can be a clean solution that support one domain ... 
%We discuss the implication on MUD standard, and various options.
%We show that currently EDNS is support by 75\%...





==> content.tex <==
\section{The problem}
The idea that the same IoT device with the same firmware demonstrates different network behavior and communicates with different domains depending on its location, was presented in our paper~\cite{IoT_MUD}.\\
The behavior of the IoT device is determined by the client registration region and not by the physical location in which the device is located.\\
NIST did not define device location as a factor that can influence the network behavior of an IoT device.\\
The MUD file is fetched by the IoT using DHCP or LLDP, and there is commonly a single MUD file for each firmware version.\\

The Network Device that implements the ACL gets the access list from the MUD Control Server, The Network Device gets the IP of the MUD Control Server from its Resolver that resolves the query by getting an answer from the vendor Authoritative Nameserver.\\
The IP of the MUD Control Server sent by the vendor Authoritative Nameserver corresponds to the Resolver IP address. But, as we say, it is a problem because we want the Network Device to get the IP of the MUD Control Server corresponding to the user registration location and not the user physical location described by the Resolver IP.

\section{Our solution}
RFC7871 describes an Extension Mechanism for client Subnet in DNS queries (ECS). \\
The RFC define an option to convey network information that is relevant to the DNS message. It carries sufficient network information about the originator for the Authoritative Nameserver to tailor responses.\\
As written in the RFC7871, the EDNS Client Subnet (ECS) option should generally be added by Recursive Resolvers when querying Authoritative Nameservers. However, the option can also be initialized by a Stub Resolver or Forwarding Resolver.\\
In our solution, the IoT device will add an EDNS Client Subnet to the DNS query that it sends to his DNS Resolver. The Client Subnet of the IoT device will correspond to the registration location defined by the user. \\
The Authoritative Nameserver of the vendor will answer the MUD URL query that the IoT device sends with the IP that correspond to the Client Subnet added to the query and not the IP of the DNS Resolver that forwards the query.\\
This way the IoT device will get the IP of the MUD Control Server that corresponds to the user registration location and get the correct MUD Policy that suits them.\\
In our case the IoT device send always the same URL query with the ECS of his registration location, and the Network Device getting the ACL that correspond to the user registration location.

